LST-1 observations of an enormous flare of BL Lacertae in 2021

The first prototype of LST (LST-1) for the Cherenkov Telescope Array has been in commissioning phase since 2018 and already started scientific observations with the low energy threshold around a few tens of GeV. In 2021, LST-1 observed BL Lac following the alerts based on multi-wavelength observations and detected prominent gamma-ray flares. In addition to the daily flux variability, LST-1 also detected sub-hour-scale intra-night variability reaching 3-4 times higher than the gamma-ray flux from the Crab Nebula above 100 GeV. In this proceeding, we will report the analysis results of LST-1 observations of BL Lac in 2021, especially focusing on flux variability.

==> LST_Authors_v2.tex <==
\tiny{\noindent
K. Abe$^{1}$,
S. Abe$^{2}$,
A. Aguasca-Cabot$^{3}$,
I. Agudo$^{4}$,
N. Alvarez Crespo$^{5}$,
L. A. Antonelli$^{6}$,
C. Aramo$^{7}$,
A. Arbet-Engels$^{8}$,
C.  Arcaro$^{9}$,
M.  Artero$^{10}$,
K. Asano$^{2}$,
P. Aubert$^{11}$,
A. Baktash$^{12}$,
A. Bamba$^{13}$,
A. Baquero Larriva$^{5,14}$,
L. Baroncelli$^{15}$,
U. Barres de Almeida$^{16}$,
J. A. Barrio$^{5}$,
I. Batkovic$^{9}$,
J. Baxter$^{2}$,
J. Becerra González$^{17}$,
E. Bernardini$^{9}$,
M. I. Bernardos$^{4}$,
J. Bernete Medrano$^{18}$,
A. Berti$^{8}$,
P. Bhattacharjee$^{11}$,
N. Biederbeck$^{19}$,
C. Bigongiari$^{6}$,
E. Bissaldi$^{20}$,
O. Blanch$^{10}$,
G. Bonnoli$^{21}$,
P. Bordas$^{3}$,
A. Bulgarelli$^{15}$,
I. Burelli$^{22}$,
L. Burmistrov$^{23}$,
M. Buscemi$^{24}$,
M. Cardillo$^{25}$,
S. Caroff$^{11}$,
A. Carosi$^{6}$,
M. S. Carrasco$^{26}$,
F. Cassol$^{26}$,
D. Cauz$^{22}$,
D. Cerasole$^{27}$,
G. Ceribella$^{8}$,
Y. Chai$^{8}$,
K. Cheng$^{2}$,
A. Chiavassa$^{28}$,
M. Chikawa$^{2}$,
L. Chytka$^{29}$,
A. Cifuentes$^{18}$,
J. L. Contreras$^{5}$,
J. Cortina$^{18}$,
H. Costantini$^{26}$,
M. Dalchenko$^{23}$,
F. Dazzi$^{6}$,
A. De Angelis$^{9}$,
M. de Bony de Lavergne$^{11}$,
B. De Lotto$^{22}$,
M. De Lucia$^{7}$,
R. de Menezes$^{28}$,
L. Del Peral$^{30}$,
G. Deleglise$^{11}$,
C. Delgado$^{18}$,
J. Delgado Mengual$^{31}$,
D. della Volpe$^{23}$,
M. Dellaiera$^{11}$,
A. Di Piano$^{15}$,
F. Di Pierro$^{28}$,
A. Di Pilato$^{23}$,
R. Di Tria$^{27}$,
L. Di Venere$^{27}$,
C. Díaz$^{18}$,
R. M. Dominik$^{19}$,
D. Dominis Prester$^{32}$,
A. Donini$^{6}$,
D. Dorner$^{33}$,
M. Doro$^{9}$,
L. Eisenberger$^{33}$,
D. Elsässer$^{19}$,
G. Emery$^{26}$,
J. Escudero$^{4}$,
V. Fallah Ramazani$^{34}$,
G. Ferrara$^{24}$,
F. Ferrarotto$^{35}$,
A. Fiasson$^{11,36}$,
L. Foffano$^{25}$,
L. Freixas Coromina$^{18}$,
S. Fröse$^{19}$,
S. Fukami$^{2}$,
Y. Fukazawa$^{37}$,
E. Garcia$^{11}$,
R. Garcia López$^{17}$,
C. Gasbarra$^{38}$,
D. Gasparrini$^{38}$,
D. Geyer$^{19}$,
J. Giesbrecht Paiva$^{16}$,
N. Giglietto$^{20}$,
F. Giordano$^{27}$,
P. Gliwny$^{39}$,
N. Godinovic$^{40}$,
R. Grau$^{10}$,
J. Green$^{8}$,
D. Green$^{8}$,
S. Gunji$^{41}$,
P. Günther$^{33}$,
J. Hackfeld$^{34}$,
D. Hadasch$^{2}$,
A. Hahn$^{8}$,
K. Hashiyama$^{2}$,
T.  Hassan$^{18}$,
K. Hayashi$^{2}$,
L. Heckmann$^{8}$,
M. Heller$^{23}$,
J. Herrera Llorente$^{17}$,
K. Hirotani$^{2}$,
D. Hoffmann$^{26}$,
D. Horns$^{12}$,
J. Houles$^{26}$,
M. Hrabovsky$^{29}$,
D. Hrupec$^{42}$,
D. Hui$^{2}$,
M. Hütten$^{2}$,
M. Iarlori$^{43}$,
R. Imazawa$^{37}$,
T. Inada$^{2}$,
Y. Inome$^{2}$,
K. Ioka$^{44}$,
M. Iori$^{35}$,
K. Ishio$^{39}$,
I. Jimenez Martinez$^{18}$,
J. Jurysek$^{45}$,
M. Kagaya$^{2}$,
V. Karas$^{46}$,
H. Katagiri$^{47}$,
J. Kataoka$^{48}$,
D. Kerszberg$^{10}$,
Y. Kobayashi$^{2}$,
K. Kohri$^{49}$,
A. Kong$^{2}$,
H. Kubo$^{2}$,
J. Kushida$^{1}$,
M. Lainez$^{5}$,
G. Lamanna$^{11}$,
A. Lamastra$^{6}$,
T. Le Flour$^{11}$,
M. Linhoff$^{19}$,
F. Longo$^{50}$,
R. López-Coto$^{4}$,
A. López-Oramas$^{17}$,
S. Loporchio$^{27}$,
A. Lorini$^{51}$,
J. Lozano Bahilo$^{30}$,
P. L. Luque-Escamilla$^{52}$,
P. Majumdar$^{53,2}$,
M. Makariev$^{54}$,
D. Mandat$^{45}$,
M. Manganaro$^{32}$,
G. Manicò$^{24}$,
K. Mannheim$^{33}$,
M. Mariotti$^{9}$,
P. Marquez$^{10}$,
G. Marsella$^{24,55}$,
J. Martí$^{52}$,
O. Martinez$^{56}$,
G. Martínez$^{18}$,
M. Martínez$^{10}$,
A. Mas-Aguilar$^{5}$,
G. Maurin$^{11}$,
D. Mazin$^{2,8}$,
E. Mestre Guillen$^{52}$,
S. Micanovic$^{32}$,
D. Miceli$^{9}$,
T. Miener$^{5}$,
J. M. Miranda$^{56}$,
R. Mirzoyan$^{8}$,
T. Mizuno$^{57}$,
M. Molero Gonzalez$^{17}$,
E. Molina$^{3}$,
T. Montaruli$^{23}$,
I. Monteiro$^{11}$,
A. Moralejo$^{10}$,
D. Morcuende$^{5}$,
A.  Morselli$^{38}$,
V. Moya$^{5}$,
H. Muraishi$^{58}$,
K. Murase$^{2}$,
S. Nagataki$^{59}$,
T. Nakamori$^{41}$,
A. Neronov$^{60}$,
L. Nickel$^{19}$,
M. Nievas Rosillo$^{17}$,
K. Nishijima$^{1}$,
K. Noda$^{2}$,
D. Nosek$^{61}$,
S. Nozaki$^{8}$,
M. Ohishi$^{2}$,
Y. Ohtani$^{2}$,
T. Oka$^{62}$,
A. Okumura$^{63,64}$,
R. Orito$^{65}$,
J. Otero-Santos$^{17}$,
M. Palatiello$^{22}$,
D. Paneque$^{8}$,
F. R.  Pantaleo$^{20}$,
R. Paoletti$^{51}$,
J. M. Paredes$^{3}$,
M. Pech$^{45,29}$,
M. Pecimotika$^{32}$,
M. Peresano$^{28}$,
F. Pfeiffle$^{33}$,
E. Pietropaolo$^{66}$,
G. Pirola$^{8}$,
C. Plard$^{11}$,
F. Podobnik$^{51}$,
V. Poireau$^{11}$,
M. Polo$^{18}$,
E. Pons$^{11}$,
E. Prandini$^{9}$,
J. Prast$^{11}$,
G. Principe$^{50}$,
C. Priyadarshi$^{10}$,
M. Prouza$^{45}$,
R. Rando$^{9}$,
W. Rhode$^{19}$,
M. Ribó$^{3}$,
C. Righi$^{21}$,
V. Rizi$^{66}$,
G. Rodriguez Fernandez$^{38}$,
M. D. Rodríguez Frías$^{30}$,
T. Saito$^{2}$,
S. Sakurai$^{2}$,
D. A. Sanchez$^{11}$,
T. Šarić$^{40}$,
Y. Sato$^{67}$,
F. G. Saturni$^{6}$,
V. Savchenko$^{60}$,
B. Schleicher$^{33}$,
F. Schmuckermaier$^{8}$,
J. L. Schubert$^{19}$,
F. Schussler$^{68}$,
T. Schweizer$^{8}$,
M. Seglar Arroyo$^{11}$,
T. Siegert$^{33}$,
R. Silvia$^{27}$,
J. Sitarek$^{39}$,
V. Sliusar$^{69}$,
A. Spolon$^{9}$,
J. Strišković$^{42}$,
M. Strzys$^{2}$,
Y. Suda$^{37}$,
H. Tajima$^{63}$,
M. Takahashi$^{63}$,
H. Takahashi$^{37}$,
J. Takata$^{2}$,
R. Takeishi$^{2}$,
P. H. T. Tam$^{2}$,
S. J. Tanaka$^{67}$,
D. Tateishi$^{70}$,
P. Temnikov$^{54}$,
Y. Terada$^{70}$,
K. Terauchi$^{62}$,
T. Terzic$^{32}$,
M. Teshima$^{8,2}$,
M. Tluczykont$^{12}$,
F. Tokanai$^{41}$,
D. F. Torres$^{71}$,
P. Travnicek$^{45}$,
S. Truzzi$^{51}$,
A. Tutone$^{6}$,
M. Vacula$^{29}$,
P. Vallania$^{28}$,
J. van Scherpenberg$^{8}$,
M. Vázquez Acosta$^{17}$,
I. Viale$^{9}$,
A. Vigliano$^{22}$,
C. F. Vigorito$^{28,72}$,
V. Vitale$^{38}$,
G. Voutsinas$^{23}$,
I. Vovk$^{2}$,
T. Vuillaume$^{11}$,
R. Walter$^{69}$,
Z. Wei$^{71}$,
M. Will$^{8}$,
T. Yamamoto$^{73}$,
R. Yamazaki$^{67}$,
T. Yoshida$^{47}$,
T. Yoshikoshi$^{2}$,
N. Zywucka$^{39}$
}\\

\tiny{\noindent
$^{1}$Department of Physics, Tokai University.
$^{2}$Institute for Cosmic Ray Research, University of Tokyo.
$^{3}$Departament de Física Quàntica i Astrofísica, Institut de Ciències del Cosmos, Universitat de Barcelona, IEEC-UB.
$^{4}$Instituto de Astrofísica de Andalucía-CSIC.
$^{5}$EMFTEL department and IPARCOS, Universidad Complutense de Madrid.
$^{6}$INAF - Osservatorio Astronomico di Roma.
$^{7}$INFN Sezione di Napoli.
$^{8}$Max-Planck-Institut für Physik.
$^{9}$INFN Sezione di Padova and Università degli Studi di Padova.
$^{10}$Institut de Fisica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology.
$^{11}$LAPP, Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS-IN2P3, Annecy.
$^{12}$Universität Hamburg, Institut für Experimentalphysik.
$^{13}$Graduate School of Science, University of Tokyo.
$^{14}$Universidad del Azuay.
$^{15}$INAF - Osservatorio di Astrofisica e Scienza dello spazio di Bologna.
$^{16}$Centro Brasileiro de Pesquisas Físicas.
$^{17}$Instituto de Astrofísica de Canarias and Departamento de Astrofísica, Universidad de La Laguna.
$^{18}$CIEMAT.
$^{19}$Department of Physics, TU Dortmund University.
$^{20}$INFN Sezione di Bari and Politecnico di Bari.
$^{21}$INAF - Osservatorio Astronomico di Brera.
$^{22}$INFN Sezione di Trieste and Università degli Studi di Udine.
$^{23}$University of Geneva - Département de physique nucléaire et corpusculaire.
$^{24}$INFN Sezione di Catania.
$^{25}$INAF - Istituto di Astrofisica e Planetologia Spaziali (IAPS).
$^{26}$Aix Marseille Univ, CNRS/IN2P3, CPPM.
$^{27}$INFN Sezione di Bari and Università di Bari.
$^{28}$INFN Sezione di Torino.
$^{29}$Palacky University Olomouc, Faculty of Science.
$^{30}$University of Alcalá UAH.
$^{31}$Port d'Informació Científica.
$^{32}$University of Rijeka, Department of Physics.
$^{33}$Institute for Theoretical Physics and Astrophysics, Universität Würzburg.
$^{34}$Institut für Theoretische Physik, Lehrstuhl IV: Plasma-Astroteilchenphysik, Ruhr-Universität Bochum.
$^{35}$INFN Sezione di Roma La Sapienza.
$^{36}$ILANCE, CNRS .
$^{37}$Physics Program, Graduate School of Advanced Science and Engineering, Hiroshima University.
$^{38}$INFN Sezione di Roma Tor Vergata.
$^{39}$Faculty of Physics and Applied Informatics, University of Lodz.
$^{40}$University of Split, FESB.
$^{41}$Department of Physics, Yamagata University.
$^{42}$Josip Juraj Strossmayer University of Osijek, Department of Physics.
$^{43}$INFN Dipartimento di Scienze Fisiche e Chimiche - Università degli Studi dell'Aquila and Gran Sasso Science Institute.
$^{44}$Yukawa Institute for Theoretical Physics, Kyoto University.
$^{45}$FZU - Institute of Physics of the Czech Academy of Sciences.
$^{46}$Astronomical Institute of the Czech Academy of Sciences.
$^{47}$Faculty of Science, Ibaraki University.
$^{48}$Faculty of Science and Engineering, Waseda University.
$^{49}$Institute of Particle and Nuclear Studies, KEK (High Energy Accelerator Research Organization).
$^{50}$INFN Sezione di Trieste and Università degli Studi di Trieste.
$^{51}$INFN and Università degli Studi di Siena, Dipartimento di Scienze Fisiche, della Terra e dell'Ambiente (DSFTA).
$^{52}$Escuela Politécnica Superior de Jaén, Universidad de Jaén.
$^{53}$Saha Institute of Nuclear Physics.
$^{54}$Institute for Nuclear Research and Nuclear Energy, Bulgarian Academy of Sciences.
$^{55}$Dipartimento di Fisica e Chimica 'E. Segrè' Università degli Studi di Palermo.
$^{56}$Grupo de Electronica, Universidad Complutense de Madrid.
$^{57}$Hiroshima Astrophysical Science Center, Hiroshima University.
$^{58}$School of Allied Health Sciences, Kitasato University.
$^{59}$RIKEN, Institute of Physical and Chemical Research.
$^{60}$Laboratory for High Energy Physics, École Polytechnique Fédérale.
$^{61}$Charles University, Institute of Particle and Nuclear Physics.
$^{62}$Division of Physics and Astronomy, Graduate School of Science, Kyoto University.
$^{63}$Institute for Space-Earth Environmental Research, Nagoya University.
$^{64}$Kobayashi-Maskawa Institute (KMI) for the Origin of Particles and the Universe, Nagoya University.
$^{65}$Graduate School of Technology, Industrial and Social Sciences, Tokushima University.
$^{66}$INFN Dipartimento di Scienze Fisiche e Chimiche - Università degli Studi dell'Aquila and Gran Sasso Science Institute.
$^{67}$Department of Physical Sciences, Aoyama Gakuin University.
$^{68}$IRFU, CEA, Université Paris-Saclay.
$^{69}$Department of Astronomy, University of Geneva.
$^{70}$Graduate School of Science and Engineering, Saitama University.
$^{71}$Institute of Space Sciences (ICE-CSIC), and Institut d'Estudis Espacials de Catalunya (IEEC), and Institució Catalana de Recerca I Estudis Avançats (ICREA).
$^{72}$Dipartimento di Fisica - Universitá degli Studi di Torino.
$^{73}$Department of Physics, Konan University.
}
